Incremental Measurement of Structural Entropy for Dynamic Graphs

Structural entropy is a metric that measures the amount of information embedded in graph structure data under a strategy of hierarchical abstracting. To measure the structural entropy of a dynamic graph, we need to decode the optimal encoding tree corresponding to the best community partitioning for each snapshot. However, the current methods do not support dynamic encoding tree updating and incremental structural entropy computation. To address this issue, we propose Incre-2dSE, a novel incremental measurement framework that dynamically adjusts the community partitioning and efficiently computes the updated structural entropy for each updated graph. Specifically, Incre-2dSE includes incremental algorithms based on two dynamic adjustment strategies for two-dimensional encoding trees, i.e., the naive adjustment strategy and the node-shifting adjustment strategy, which support theoretical analysis of updated structural entropy and incrementally optimize community partitioning towards a lower structural entropy. We conduct extensive experiments on 3 artificial datasets generated by Hawkes Process and 3 real-world datasets. Experimental results confirm that our incremental algorithms effectively capture the dynamic evolution of the communities, reduce time consumption, and provide great interpretability.

==> 9-1dSE.tex <==
An information system is a system composed of many objects and the movement and interaction of these objects. 
The intuitive mathematical model of an information system is a weighted directed graph (Definition~\ref{def:wdg}).

\begin{definition}[Information System Represented by Weighted Directed Graphs]
An information system is a weighted directed graph $G = (\mathcal{V},\mathcal{E}, f)$, which satisfies the following properties:
\begin{enumerate}[(1)]
    \item $\mathcal{V} = \{v_1, v_2, ..., v_N\}$ is the node set, in which each node denotes an object;
    \item $\mathcal{E}$ denotes the set of directed edges $e = (v_i, v_j)$;
    \item for each edge $e = (v_i, v_j) \in \mathcal{E}$, $f(e) = f(v_i, v_j) >0$ is named the interactive profile from $v_i$ to $v_j$. Here, the interactive profile $f(e) = f(v_i, v_j)$ intuitively represents the influence, similarity, or probability of movement from $v_i$ to $v_j$. For $e = (v_i, v_j) \notin \mathcal{E}$, we denote $f(e) = f(v_i, v_j) = 0$.
\end{enumerate}
% by an adjacency matrix $\mathbf{A}\in \mathbb{R}^{N\times N}_{\ge 0}$, where 
\label{def:wdg}
\end{definition}

% Let $\mathbf{A}$ denote the 
Given an information system $G = (\mathcal{V},\mathcal{E}, f)$, we fix the nodes in $\mathcal{V}$ in an order like $v_1, v_2, ..., v_N$.
For $i,j \in \{1,2,..,N\}$, we define $a_{ij} = f(v_i, v_j)$.
Then we can obtain a non-negative matrix $\mathbf{A} = (a_{ij})$, named as a matrix of $G$ and denoted by $\mathbf{A}_G$.
Therefore, we give another definition for information systems as follows.

\begin{definition}[Information System Represented by Non-Negative Matrix]
An information system is an $N\times N$ non-negative matrix $\mathbf{A} = (a_{ij})$, where for each $i$ and $j \in \{1,2,...,N\}$, $a_{ij}\ge 0$.
It can also be denoted by $\mathbf{A}\in \mathbb{R}^{N\times N}_{\ge 0}$.
\label{def:matrix}
\end{definition}

\subsection{Definition of One-Dimensional Structural Entropy}

For direct graphs, the structural entropy is an uncertainty measurement defined on strongly connected graphs whose matrices must be irreducible (Definition~\ref{def:im}).

\begin{definition}[Irreducible Matrix]
Given a non-negative matrix $\mathbf{A}\in \mathbb{R}^{N\times N}_{\ge 0}$, if there exists a permutation matrix $\mathbf{P}$ such that 
\begin{equation}
    \mathbf{P} \mathbf{A} \mathbf{P} = 
    \begin{bmatrix}
        \mathbf{X} & \mathbf{Y} \\
        \mathbf{0} & \mathbf{Z}
    \end{bmatrix},
\end{equation}
where $\mathbf{X}$ and $\mathbf{Z}$ are square matrices, then $\mathbf{A}$ is said to be a reducible matrix, otherwise $\mathbf{A}$ is an irreducible matrix.
\label{def:im}
\end{definition}

Normalize each row in an irreducible $\mathbf{A}$, i.e., for each $i$ and $j$, let 
\begin{equation}
    b_{ij} = \frac{a_{ij}}{\sum_{k = 1}^N a_{ik}}.
\end{equation}
Then we can get a normalized irreducible matrix $\mathbf{B} = (b_{ij})$ where the sum of elements in each row is $1$.
There is a fundamental theorem for normalized irreducible matrices like $\mathbf{B}$:
\begin{theorem}[Perron Forbenius]
If $\mathbf{B}\in \mathbb{R}^{N\times N}_{\ge 0}$ is an irreducible matrix where for each $i$, $\sum_{k=1}^N b_{ik}= 1$, then
\begin{enumerate}[(1)]
    \item the maximum eigenvalue of $\mathbf{B}$ is $1$;
    \item the maximum eigenvalue of $\mathbf{B}$ has a unique left eigenvector;
    \item The unique left eigenvector of the maximum eigenvalue of $\mathbf{B}$ is a probability distribution, denoted by $\pi = [\pi_1, \pi_2, ..., \pi_N]$.
\end{enumerate}
\label{the:pf}
\end{theorem}

According to Theorem~\ref{the:pf}, the stationary distribution of $\mathbf{A}$ can then be defined in Definition~\ref{def:sd}.

\begin{definition}[Stationary Distribution]
Let $\mathbf{A}\in \mathbb{R}^{N\times N}_{\ge 0}$ be an irreducible matrix and $\mathbf{B}$ represents the normalized matrix of $\mathbf{A}$ where for each $i$, $\sum_{k=1}^N b_{ik}= 1$.
The stationary distribution of $\mathbf{A}$ is defined as the unique left eigenvector of the maximum eigenvalue of $\mathbf{B}$, denoted by $\pi = [\pi_1, \pi_2, ..., \pi_N]$.
\label{def:sta}
\end{definition}

Finally, the one-dimensional structural entropy (Definition~\ref{def:1dSE}) of an irreducible non-negative matrix is defined as the Shannon entropy of the stationary distribution, which measures the total amount of uncertainty embedded in the information system.

\begin{definition}[One-Dimensional Structural Entropy]
Let $\mathbf{A}\in \mathbb{R}^{N\times N}_{\ge 0}$ be an irreducible matrix and $\pi = [\pi_1, \pi_2, ..., \pi_N]$ is the stationary distribution of $\mathbf{A}$.
The one-dimensional structural entropy is defined as 
\begin{equation}
\mathcal{H}^1(\mathbf{A}) = -\sum_{i=1}^N \pi_i \log_2 \pi_i.
\label{eq:1dSE}
\end{equation}
\label{def:1dSE}
\end{definition}




\subsection{Incremental Measurement of One-Dimensional Structural Entropy}

Generally, the exact value of one-dimensional structural entropy can be obtained by Eq.~(\ref{eq:1dSE}) in $O(n)$ given the stationary distribution.
However, the calculation of the exact stationary distribution $\pi$ needs to solve the eigenvectors of $\mathbf{B}$, which usually costs $O(n^3)$.
According to Definition~\ref{def:sd}, we have
\begin{equation}
    \pi \mathbf{B} = \pi.
\end{equation}
In dynamic scenarios, the information system evolves as time passes by.
Formally, we define $\mathbf{A}_0$ as the original information system and $\mathbf{A}_1, \mathbf{A}_2,..., \mathbf{A}_T$ as the updated information systems at time $t = 1,2,...,T$.
At each time $t>0$, there exists an incremental matrix $\Delta \mathbf{A}_t$ which satisfies $\mathbf{A}_t = \mathbf{A}_{t-1} + \Delta \mathbf{A}_t$.
% Let $\mathbf{B}_t$ denote the normalized matrix of $\mathbf{A}_t$.
% Given $\Delta \mathbf{A}_t$, the updated normalized matrix $\mathbf{B}_t$ can be obtained by
% \begin{equation}
% \begin{aligned}
%     \mathbf{B}_t &= \mathbf{B}_{t-1}.
% \end{aligned}
% \end{equation}
When an information system represented by an irreducible matrix $\mathbf{A}\in \mathbb{R}^{N\times N}_{\ge 0}$ gets an incremental $\Delta \mathbf{A}$, it becomes an updated irreducible matrix $\mathbf{A}' = \mathbf{A} + \Delta \mathbf{A}$.
Let $n = ||\Delta \mathbf{A}||_0$ denote the incremental size.
Let $\mathbf{B}$ and $\mathbf{B}'$ be the normalized matrices of $\mathbf{A}$ and $\mathbf{A}'$.
Define $\Delta \mathbf{B} = \mathbf{B}' - \mathbf{B}$.
We can calculate $\Delta \mathbf{B}$ from $\mathbf{A}$ and $\Delta \mathbf{A}$ by
\begin{equation}
\Delta b_{ij} = b'_{ij} - b_{ij} = \frac{a'_{ij}}{\sum_{k=1}^{N} a'_{ik}} - \frac{a_{ij}}{\sum_{k=1}^{N} a_{ik}} = \frac{a_{ij} + \Delta a_{ij}}{(\sum_{k=1}^{N} a_{ik} + \Delta a_{ik})} - \frac{a_{ij}}{\sum_{k=1}^{N} a_{ik}}.
\end{equation}
Since a non-zero element of $\Delta \mathbf{A}$ may influence at most all $N$ elements of a row in $\mathbf{B}$, $||\Delta \mathbf{B}||_0$, named as the normalized incremental size, will be no more than $nN$.
In addition, the number of the influenced rows in $\mathbf{B}$, denoted by $n_B$, will be no more than $n$.
In the following, three ways are listed to compute the updated one-dimensional structural entropy:

\textbf{Exact value calculation by definition.}
The first way is to calculate the exact value of the updated one-dimensional structural entropy by Definition~\ref{def:sta} and~\ref{def:1dSE}.
Specifically, the new exact stationary distribution $\pi'$ is first computed by solving the left eigenvector of $\mathbf{B}'$.
The updated one-dimensional structural entropy can then be calculated by
\begin{equation}
\mathcal{H}^1(\mathbf{A'}) = -\sum_{i=1}^N \pi'_i \log_2 \pi'_i.
\label{eq:updated-1dse}
\end{equation}
Generally, the total time complexity of this way is $O(N^3)$.

\textbf{Approximate value calculation by iteration.}
In this way, we first compute the approximate stationary distribution by iteratively right-multiplying $\mathbf{A}'$, i.e.,
\begin{equation}
\pi^{(\theta)} = \pi \mathbf{B}'^\theta = \pi (\mathbf{B} +\Delta \mathbf{B})^\theta,
\label{eq:theta-pi}
\end{equation}
where $\theta \in \mathbb{N}$ is the iteration number.
Next, we compute the Shannon entropy of $\pi^{\theta}$ as the approximate one-dimensional structural entropy:
\begin{equation}
\mathcal{H}^1(\mathbf{A'}) \approx -\sum_{i=1}^N \pi^{(\theta)}_i \log_2 \pi^{(\theta)}_i.
\end{equation}
The total computational complexity of this way is about $O(\theta N^2)$.

\textbf{Fast approximate value calculation.}
In this part, we propose a new method for fast approximation of updated one-dimensional structural entropy with low time complexity.
The key idea is to reduce the redundancy of matrix multiplication in Eq.~(\ref{eq:theta-pi}).
In particular, when $\theta = 1$, Eq.~(\ref{eq:theta-pi}) can be expanded as follows:
\begin{equation}
\begin{aligned}
    \pi^{(1)} &= \pi (\mathbf{B} +\Delta \mathbf{B})\\
    &=\pi + \pi \Delta \mathbf{B}\\
    &=\pi + [\sum_{i=1}^{N} \pi_i \Delta b_{i1}, \sum_{i=1}^{N} \pi_i \Delta b_{i2}, ..., \sum_{i=1}^{N} \pi_i \Delta b_{iN}].
\end{aligned}
\label{eq:exp1-theta-pi}
\end{equation}
Let $\mathcal{X}$ denote the indices of all non-zero rows in $\Delta \mathbf{B}$.
Eq.~(\ref{eq:exp1-theta-pi}) can then be reduced to
\begin{equation}
\begin{aligned}
    \pi^{(1)} &= \pi + [\sum_{x\in \mathcal{X}} \pi_x \Delta b_{x1}, \sum_{x\in \mathcal{X}} \pi_x \Delta b_{x2}, ..., \sum_{x\in \mathcal{X}} \pi_x \Delta b_{xN}]\\
    &= \pi + \sum_{x\in \mathcal{X}} \pi_x [\Delta b_{x1}, \Delta b_{x2}, ..., \Delta b_{xN}],
\end{aligned}
\label{eq:exp2-theta-pi}
\end{equation}
and
\begin{equation}
\begin{aligned}
    \pi^{(1)}_i &= \pi_i + \sum_{x\in \mathcal{X}} \pi_x \Delta b_{xi}.
\end{aligned}
\end{equation}





==> minor-revision.tex <==


Ms. Ref. No.: ARTINT-D-23-00582R1
Title: Incremental Measurement of Structural Entropy for Dynamic Graphs
Artificial Intelligence

Dear Hao,

I attach reviews of the above paper that you submitted to 'Artificial Intelligence' for publication. I accept it for publication subject to you addressing all the points raised in the reviews and you fulfilling m request below. Your revision will not be sent out for a second review, but will be checked by the Associate Editor handling the paper.

In addition to the comments below, since you added a new author during the review process, I am thereby asking you to add a letter **signed by all authors** stating:
a) exactly what is the contribution of the new author to the paper (not in vague terms like data curation, but in terms of the changes that were made between the initial version and R1)
b) and stating that all authors agree with the addition of this author and current order of authors.

If you submit a revised manuscript, please also:

a) outline each change made (point by point) as raised in the reviewer comments

 AND/OR

b) provide a suitable rebuttal to each reviewer comment not addressed

c) upload all source files of the revision.

To submit your revision, please do the following:

1. Go to: https://www.editorialmanager.com/artint/

2. Enter your login details

3. Click [Author Login]
This takes you to the Author Main Menu.

4. Click [Submissions Needing Revision]


The revised version of your submission is due by Jun 29, 2024.

I look forward to receiving your revised manuscript.

Yours sincerely,

Sylvie Thiebaux
Editor-in-Chief
Artificial Intelligence


REVIEWERS' COMMENTS:

The reviewers agree that the authors have addressed most issues raised in the last review cycle. They also indicate that the following minor issues should be addressed before publication:
- Discuss the limitation related to the Leiden results (R1)
- Add more explanations on global invariant / local difference and node-shifting adjustment strategy (R2)
~~~~~~~~~~~~~~~~~~~~

Reviewer #1: The authors conducted a good-faith revision in response to my reviews. Their revision report is detailed, and the revisions to the paper are significant. I only have one minor concern about the effect of the static community detection methods. In the revised version, the authors explained well why the results of Leiden were different from those of the other methods and made the results consistent with those of the other methods by changing the objective function. However, this modification requires a "detailed analysis," which will bring in additional costs and reduce the utility of the proposed method in real-world applications. I suggest the authors discuss this limitation in the discussion section.



Reviewer #3: The authors have addressed my concerns. I am happy to recommend acceptance.


Reviewer #5: Thank you for the reply. There are still a couple of questions:

1. It would be better to highlight the sense of introducing global invariant / local difference at the beginning of Section 3.1.2, which would make its relationship to Section 3.1.1 clearer to the reader. The current structure is somewhat confusing.
2. Since global invariant and local difference are based on approximation, is there a gap between Incre-2dSE and current static algorithms [1]? Additionally, does this gap accumulate over time as the graph is updated?
3. Can node-shifting adjustment strategy overcome the limits of naive adjustment strategy listed in Section 3.1.5? In node-shifting adjustment strategy, how do you choose the maximum number of iterations?

[1] A. Li, Y. Pan, Structural information and dynamical complexity of networks, IEEE Transactions on Information Theory 62 (6) (2016) 3290-3339.

==> revision_plan.tex <==
Revision Plan (11.6 - 11.30, 25 days, 18 work days)

1. Writing (6 days)
1.1 minor revisions
1.2 A broader discussion between two strategies
1.3 Means of boundedness analysis and convergence analysis

2. Experiment (12 days)
2.1 Threshold to boost efficiency (2 days) 
Finished.

2.2 Detailed Hawkes Process (5 days)
details are added.

2.3 Bigger dataset to evaluate time consumption (3 days)

2.4 Additional parameter analysis (2 days)

11.25-27--2.3+2.4 code/exp
11.28-30--writing

11/29 exp remain
1. exp1 finish (only new hawkes left) & draw
2. noise hawkes generate
3. noise analysis (exp4) & draw
offline - do exps

11/30
finish the remained exp -- to reply Peng
full-time reading the interview paper
**Change the dataset -> dblp
**Change the static -> label propagation? can be better?

12/1-12/3
write paper 1h
rebuttal 1h
read interview paper 1h

12/4
interview 1h
write paper 1h
rebuttal 1h


-------------------------------------------------
20 days revision plan (60h)

1. 实现local pagerank策略下的一维结构熵增量度量（10days）30h
首先编程实现，然后做实验demo，最后写文章。
随机衰减策略/百分比阈值策略

2. 实现多初始场景下（如随机块）的初始图的hawkes过程并进行实验（5days）15h

3. 全文统修（5days）15h

预计2月8日完工




